DeCo: Decoupling Token Compression from Semantic Abstraction in Multimodal Large Language Models

The visual projector, which bridges the vision and language modalities and facilitates cross-modal alignment, serves as a crucial component in MLLMs. However, measuring the effectiveness of projectors in vision-language alignment remains under-explored, which currently can only be inferred from the performance of MLLMs on downstream tasks. Motivated by the problem, this study examines the projector module by interpreting the vision-language semantic flow within MLLMs. Specifically, we trace back the semantic relevance flow from generated language tokens to raw visual encoder patches and the intermediate outputs produced by projectors. Our findings reveal that compressive projectors (e.g., QFormer), abstract visual patches into a limited set of semantic concepts, such as objects or attributes, resulting in a 'double abstraction' phenomenon. This involves a first visual semantic abstraction by the projector referring to pre-defined query tokens, and a second extraction by the LLM based on text instructions. The double abstraction is inefficient in training and will result in cumulative vision semantics deficiency. To mitigate this issue, we propose the key insight of 'Decouple Compression from Abstraction (DeCo), that is compressing the visual token number at the patch level by projectors and allowing the LLM to handle visual semantic abstraction entirely. Consequently, we adopt a simple compressor, i.e., 2D Adaptive Pooling, to downsample visual patches in a parameter-free manner. Empirical evaluation demonstrates that DeCo surpasses traditional compressive projectors regarding both performance and efficiency. It achieves performance gains of 0.9%, 7.1%, and 2.9% across the MLLM Benchmarks, Visual Localization, and Open-ended VQA tasks with fewer trainable parameters and faster convergence speed.

==> tables/main_locality.tex <==
% \begin{wraptable}{r}{0.6\textwidth}
\begin{table}[t]
\centering
\caption{
\small
Vision spatial understanding capability across different projectors. % \#V denotes the number of visual tokens after projection. 
Task names are abbreviated as follows: Position (POS) for MME~\cite{fu2023mme}, Spatial Relationship (SR), Object Localization (OL), and Physical Relation (PR) for MMBench~\cite{ge2024mllmbench}, and Spatial Relation (SR) and Instance Location (IL) for SEED-Bench~\cite{li2023seedbench}.}
\label{tab:main_locality}
\centering
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{l c cccccc c}
\toprule
\multirow{2}{*}{Projector} &
  \multirow{2}{*}{\#V} &
  \multicolumn{1}{c}{MME} &
  \multicolumn{3}{c}{MMB} &
  \multicolumn{2}{c}{SEED} &
  \multirow{2}{*}{Avg}  \\
  \addlinespace[2pt] \cmidrule(lr){3-3} \cmidrule(lr){4-6} \cmidrule(lr){7-8} \addlinespace
 &
   &
  \multicolumn{1}{l}{POS} &
  \multicolumn{1}{l}{SR} &
  \multicolumn{1}{l}{OL} &
  \multicolumn{1}{l}{PR} &
  \multicolumn{1}{l}{SR} &
  \multicolumn{1}{l}{IL} &   \\ \midrule
\demph{Linear~\cite{liu2023llava15}}       & \demph{576} & \demph{123.3}          & \demph{20.0}          & \demph{51.9}          & \demph{33.3}          & \demph{50.2}          & \demph{59.6}  &  \demph{56.4}       \\ \midrule
QFormer~\cite{li2023blip2}      & 144 & 73.3           & 17.8          & 33.3          & 33.3          & 39.0         & 48.9    &  40.9   \\
C-Abstractor~\cite{cha2023honeybee} & 144 & 116.7          & 15.6          & 42.0          & \textbf{54.2} & 43.5          & 54.4      & 54.4   \\
% D-Abstractor~\cite{cha2023honeybee} & 144 & 126.7 &        20.0 & 43.2 &	37.5&	44.4 &	55.4       \\
% MaxPooling &  &          &          &           &  &           &          \\


\model (Ours)         & 144 & \textbf{116.7} & \textbf{24.4} & \textbf{48.1} & 41.7          & \textbf{46.6} & \textbf{58.5} & \textbf{56.0} \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
